Dark Side Augmentation: Generating Diverse Night Examples for Metric Learning

Image retrieval methods based on CNN descriptors rely on metric learning from a large number of diverse examples of positive and negative image pairs. Domains, such as night-time images, with limited availability and variability of training data suffer from poor retrieval performance even with methods performing well on standard benchmarks. We propose to train a GAN-based synthetic-image generator, translating available day-time image examples into night images. Such a generator is used in metric learning as a form of augmentation, supplying training data to the scarce domain. Various types of generators are evaluated and analyzed. We contribute with a novel light-weight GAN architecture that enforces the consistency between the original and translated image through edge consistency. The proposed architecture also allows a simultaneous training of an edge detector that operates on both night and day images. To further increase the variability in the training examples and to maximize the generalization of the trained model, we propose a novel method of diverse anchor mining. The proposed method improves over the state-of-the-art results on a standard Tokyo 24/7 day-night retrieval benchmark while preserving the performance on Oxford and Paris datasets. This is achieved without the need of training image pairs of matching day and night images. The source code is available at https://github.com/mohwald/gandtr .

==> fig/cyclegan-model.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{img/cyclegan-model.pdf}
    \caption[Night generator training.]{The pass of a day image (up left) through the CycleGAN architecture during one training step. After passing through both generators, the resulting image (up right) is compared to the input in L1 norm to ensure consistency. The night discriminator predicts whether the intermediate translated image (up center) and the input night image (bottom left) are real or fake. Only one direction of the CycleGAN architecture is displayed.}
    %-- the pass of a night image is analogous, with the order of generators swapped and the night discriminator replaced by a day discriminator.}
   \label{fig:cyclegan-model}
\end{figure}

==> fig/outputs.tex <==
\begin{figure}[t]
\newcommand{\outscale}{0.19}
\newcommand{\toplab}[1]{\parbox{\outscale\linewidth}{\centering \scriptsize #1}}
\newcommand{\subfloat}[1]{\parbox{\outscale\linewidth}{\includegraphics[width=\linewidth]{#1}}}
\newcommand{\hspacing}{\hspace{1.5em}}

  \centering
   \toplab{Original}  \toplab{GAN}  \toplab{DRIT}  \toplab{CUT}  \toplab{\hedn GAN}\\
    %{\tiny \hspace{0.1em} Original \hspace{2.5em} GAN \hspace{1.6em} GAN Aachen \hspace{1.6em} DRIT \hspace{1.6em} CUT \hspace{1.6em} HED-GAN \hspace{3.5em} Original \hspace{2.5em} GAN \hspace{1.6em} GAN Aachen \hspace{1.6em} DRIT \hspace{1.6em} CUT \hspace{1.6em} HED-GAN \hspace{0.5em}} ~ \\[0.4em]
    \subfloat{img/output/input/67.jpg} 
    \subfloat{img/output/sfm/new67.jpg} 
%    \subfloat{img/output/aachen/new67.jpg} 
    \subfloat{img/output/drit/67.jpg} 
    \subfloat{img/output/cut/67.jpg} 
    \subfloat{img/output/hed/67.jpg} \\
    \subfloat{img/output/input/26.jpg} 
    \subfloat{img/output/sfm/new26.jpg} 
%    \subfloat{img/output/aachen/new26.jpg} 
    \subfloat{img/output/drit/26.jpg} 
    \subfloat{img/output/cut/26.jpg} 
    \subfloat{img/output/hed/26.jpg} \\
    \subfloat{img/output/input/4.jpg} 
    \subfloat{img/output/sfm/new4.jpg} 
%    \subfloat{img/output/aachen/new4.jpg} 
    \subfloat{img/output/drit/4.jpg} 
    \subfloat{img/output/cut/4.jpg} 
    \subfloat{img/output/hed/4.jpg} \\
    \subfloat{img/output/input/11.jpg} 
    \subfloat{img/output/sfm/new11.jpg} 
 %   \subfloat{img/output/aachen/new11.jpg} 
    \subfloat{img/output/drit/11.jpg} 
    \subfloat{img/output/cut/11.jpg} 
    \subfloat{img/output/hed/11.jpg}
    \\\vspace{1em}
    \caption{Examples of day-to-night translations with various generators. Each row consists of (left to right) the source image, and images translated by: CycleGAN, DRIT, CUT, and the proposed HED\textsuperscript{N}GAN. All models are trained on the SfM dataset.}
   \label{fig:outputs}
\end{figure}

==> tab/rebuttal.tex <==
% \begin{table}[t] \centering
% \newcommand{\firstsup}[1]{{\bf #1}}
% % \newcommand{\secondsup}[1]{{\bf #1}}
% \begin{tabular}{|l||r|r|} \hline % 0f01
%     Method & Recall@(1/5/10) & mAP@(1/5/10) \\\hline\hline
%     GeM	& 34.7 / 45.8 / 50.7 & 34.7 / 24.1 / 21.4 \\\hline
%     GeM N/D \nddata & 31.7 / 42.9 / 47.1 & 31.7 / 22.1 / 19.6 \\\hline
%     CycleGAN \clahe \diverse & 35.3 / \firstsup{47.1} / \firstsup{51.6} & 35.3 / 24.8 / 20.5 \\\hline
%     \hedn GAN \clahe \diverse & \firstsup{36.4} / 46.3 / 49.9 & \firstsup{36.4} / \firstsup{25.0} / \firstsup{22.2} \\\hline
%
% \end{tabular}\\[3pt]
 %    \caption{Evaluation of baseline and our methods on MSLS test dataset \cite{warburg2020msls}. All methods are evaluated only on single view task (im2im), where overall top-1/5/10 recall and mean average precision (mAP) are reported in \%.
%     All methods are described the same way as in the Table~1 in the paper.
%     % All methods were trained on \textit{SfM} dataset, while the method of \cite{jenicek} marked with \nddata was trained on \textit{SfM-N/D} dataset.
%     % All methods were trained on \textit{SfM} dataset using annotations from 3D reconstructions with unpaired day-night images, while the method of \cite{jenicek} marked with \nddata was trained on \textit{SfM-N/D} with paired day-night images.
%     The best score is in bold.
%     \vspace{-1.5em}}
% \label{tab:msls}
% \end{table}

% | Dataset : Subtask : Model                  | Recall@1 | Recall@5 | Recall@10 | Recall@20 | map@1 | map@5 | map@10 | map@20 |
% | ------------------------------------------ | -------- | -------- | --------- | --------- | ----- | ----- | ------ | ------ |
% | test:all:vgg16 GeM                         | 0.347    | 0.458    | 0.507     | 0.557     | 0.347 | 0.241 | 0.214  | 0.201  |
% | test:all:vgg16 GeM N/D                     | 0.317    | 0.429    | 0.471     | 0.519     | 0.317 | 0.221 | 0.196  | 0.183  |
% | test:all:vgg16_tpami18_e40:clahe           | 0.339    | 0.453    | 0.504     | 0.554     | 0.339 | 0.236 | 0.210  | 0.198  |
% | test:all:vgg16_iccv19_clahe_sfmnd:camready | 0.320    | 0.416    | 0.466     | 0.511     | 0.320 | 0.217 | 0.190  | 0.179  |
% | test:all:vgg16 CycleGAN                    | 0.353    | 0.471    | 0.516     | 0.569     | 0.353 | 0.248 | 0.220  | 0.205  |
% | test:all:vgg16 HEDnGAN                     | 0.364    | 0.463    | 0.499     | 0.551     | 0.364 | 0.250 | 0.222  | 0.209  |

\begin{table}[t] \centering
\newcommand{\firstsup}[1]{{\bf #1}}
% \newcommand{\secondsup}[1]{{\bf #1}}
\setlength{\tabcolsep}{0.4em}
{\small 
\begin{tabular}{|l||r|r|r|} \hline % 0f01
    Method & top-1 & w/o global map & with global map \\\hline\hline
    GeM	& 0 / 0 /16.2 & 59.2 / 73.8 / 87.4 & 62.3 / 76.4 / 91.1 \\\hline
    CycleGAN \clahe \diverse & 0 / 0 / \firstsup{18.8} & 61.3 / 78.0 / \firstsup{90.6} & 62.8 / 78.5 / 92.1 \\\hline
    \hedn GAN \clahe \diverse & 0 / 0 / 18.3 & \firstsup{62.3} / \firstsup{79.1} / 90.1 & 62.8 / 78.5 / 92.1 \\\hline
    R-GeM & 0 / 0.5 / 16.8 & 60.7 / 75.4 / 88.0 & 62.8 / 79.1 / 90.6 \\
    R-CycleGAN & 0 / 0.5 / 20.4 & 63.4 / 77.0 / 92.1 & 66.0 / 80.6 / 95.8 \\
    R-\hedn GAN & 0 / 0.5 / 19.4 & 64.9 / 79.6 / 94.2 & 65.4 / 80.6 / 94.2 \\\hline
%     AP-GeM & 0 / 0.0 / 17.3 & 63.9 / 79.6 / 94.8 & 68.6 / 83.8 / 96.9 \\\hline

\end{tabular}}\\[3pt]
    \caption{Aachen v1.1 night.}
    \vspace{-0.5em}
\label{tab:aachen}
\end{table}

\begin{table}[t] \centering
\newcommand{\firstsup}[1]{{\bf #1}}
% \newcommand{\secondsup}[1]{{\bf #1}}
\setlength{\tabcolsep}{0.4em}
{\small
\begin{tabular}{|l||r|r|r|} \hline % 0f01
    Method & top-1 pose & w/o global map & with global map \\\hline\hline
    GeM	& 0.0 / 0.6 / 7.1 & 5.9 / 11.4 / 16.1 & 8.2 / 14.6 / 20.3 \\\hline
    CycleGAN \clahe \diverse & 0.1 / 1.3 / \firstsup{17.4} & \firstsup{12.2} / 21.9 / 29.2 & \firstsup{14.5} / 26.1 / 35.6 \\\hline
    \hedn GAN \clahe \diverse & 0.1 / 1.3 / 16.3 & 12.1 / \firstsup{22.7} / \firstsup{31.1} & 14.0 / \firstsup{27.1} / \firstsup{37.8} \\\hline
    R-GeM & 0.1 / 0.9 / 10.1 & 7.6 / 14.6 / 20.3 & 10.3 / 18.1 / 25.2 \\
    R-CycleGAN & 0.5 / 2.2 / 22.6 & 14.1 / 26.2 / 36.0 & 16.3 / 29.2 / 40.9 \\
    \hedn GAN & 0.3 / 1.7 / 21.4 & 13.4 / 24.7 / 34.3 & 15.9 / 29.7 / 40.0 \\\hline
%     AP-GeM & 0.5 / 3.0 / 28.4 & 19.1 / 36.4 / 53.4 & 21.1 / 40.3 / 58.3 \\\hline

\end{tabular}}\\[3pt]
    \caption{RobotCar Seasons v1 night.}
    \vspace{-1.5em}
\label{tab:robotcar}
\end{table}

